Newton's methods for solving linear inverse problems with neural network coders

Neural networks functions are supposed to be able to encode the desired solution of an inverse problem very efficiently. In this paper, we consider the problem of solving linear inverse problems with neural network coders. First we establish some correspondences of this formulation with existing concepts in regularization theory, in particular with state space regularization, operator decomposition and iterative regularization methods. A Gauss-Newton's method is suitable for solving encoded linear inverse problems, which is supported by a local convergence result. The convergence studies, however, are not complete, and are based on a conjecture on linear independence of activation functions and its derivatives.

==> Makefile <==
MAIN = HofSch23

.PHONY: default full final clean check whoareyou help

default:
	pdflatex --file-line-error $(MAIN).tex

full:
	latexmk -pdf --file-line-error $(MAIN).tex

final:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex
	biber --output_format=bibtex --output_resolve $(MAIN) -O biber.bib
	#sed $(MAIN).tex -e '/^\\def\\notfinal{}/d' > $(MAIN)_final.tex
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN)_final.tex
	latexmk -c $(MAIN).tex
	latexmk -c $(MAIN)_final.tex

clean:
	latexmk -c $(MAIN).tex
	rm -f $(MAIN).bbl $(MAIN).run.xml $(MAIN).thm $(MAIN).pdf

check:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex

whoareyou:
	@echo $(MAIN)

bib:
	$(eval AUX := $(shell mktemp -d))
	latexmk -gg -pdf -jobname=extract -pdflatex="/usr/bin/pdflatex --file-line-error --shell-escape --synctex=1 %O '\def\extract{}\input{%S}'" -output-directory=${AUX} ${MAIN}.tex
	biber --output_format=bibtex --output_resolve -O ${AUX}/extract.bib ${AUX}/extract
	echo "\n%% Warning: This file is autogenerated, editing might be futile.\n" > csc.bib
	cat ${AUX}/extract.bib >> csc.bib

help:
	@echo ""
	@echo "make targets are:"
	@echo ""
	@echo "  default (default):"
	@echo "    just builds the tex file (without bibliography)"
	@echo ""
	@echo "  bib:"
	@echo "    extracts bibliography to bib.bib"
	@echo ""
	@echo "  full:"
	@echo "    builds the tex file (with bibliography)"
	@echo ""
	@echo "  final:"
	@echo "    extracts the bibliography into a local bib file"
	@echo "    creates an $(MAIN)_final.tex file using the extracted bib data"
	@echo ""
	@echo "  clean:"
	@echo "    cleans up temporary files"
	@echo ""
	@echo "  (check):"
	@echo "    used by the papercheck deamon, same as full but doesn't halt on error"
	@echo ""
	@echo "  (whoareyou):"
	@echo "    used by the papercheck daemon to identify this Makefile"
	@echo ""


